Explore Theory of Mind: Program-guided adversarial data generation for theory of mind reasoning

Do large language models (LLMs) have theory of mind? A plethora of papers and benchmarks have been introduced to evaluate if current models have been able to develop this key ability of social intelligence. However, all rely on limited datasets with simple patterns that can potentially lead to problematic blind spots in evaluation and an overestimation of model capabilities. We introduce ExploreToM, the first framework to allow large-scale generation of diverse and challenging theory of mind data for robust training and evaluation. Our approach leverages an A* search over a custom domain-specific language to produce complex story structures and novel, diverse, yet plausible scenarios to stress test the limits of LLMs. Our evaluation reveals that state-of-the-art LLMs, such as Llama-3.1-70B and GPT-4o, show accuracies as low as 0% and 9% on ExploreToM-generated data, highlighting the need for more robust theory of mind evaluation. As our generations are a conceptual superset of prior work, fine-tuning on our data yields a 27-point accuracy improvement on the classic ToMi benchmark (Le et al., 2019). ExploreToM also enables uncovering underlying skills and factors missing for models to show theory of mind, such as unreliable state tracking or data imbalances, which may contribute to models' poor performance on benchmarks.

==> sections/abstract.tex <==
% However, all rely on simple patterns that can potentially lead to overestimating model abilities, with concerns of benchmarks having blind spots and existing models overfitting to them.

\begin{abstract}
% Theory of Mind (ToM) is a crucial aspect of social intelligence, yet large language models (LLMs) struggle to demonstrate robust ToM reasoning skills.
Do large language models (LLMs) have theory of mind? A plethora of papers~and benchmarks have been introduced to evaluate if current models have been able to develop this key ability of social intelligence. However, all rely on limited datasets with simple patterns that can potentially lead to problematic blind spots in evaluation and an overestimation of model capabilities. %, with concerns about existing models overfitting to these benchmarks, despite their problematic blind spots.}
%
%\yejin{CHANGE The result is papers claiming models can reason about social contexts while our everyday lived experience demonstrates otherwise.} 
%\editmel{However, all rely on simple patterns that can potentially lead to overestimation of model capabilities, }
%\editmel{with concerns that these benchmarks contain problematic blind spots and existing models are overfitting to them.} %%% existing llms quickly saturate benchmarks; despite existing concerns there are blind spot in evaluation
%\editmel{There has been concerns of benchmarks having blind spots and existing models overfitting to them.} %%% existing llms quickly saturate benchmarks; despite existing concerns there are blind spot in evaluation
%For this reason, we introduce 
We introduce \methodname{}, the first framework to allow large-scale generation of diverse and challenging theory of mind data for robust training and evaluation.
%Reasoning about the mental states of other people---known as Theory of Mind (ToM)---is a key aspect of social intelligence. Nonetheless, despite their continuously growing performance and their deployment in user facing-settings, large language models (LLMs) struggle to demonstrate robust theory of mind reasoning skills, and faithful evaluation remains challenging: existing benchmarks are limited in scale and diversity, and often overestimate models' capabilities. We introduce \methodname{}, a novel framework that generates diverse, challenging, and scalable theory of mind data that can be used for both training and evaluation. 
%Our approach leverages a custom domain-specific language and A* search to produce story structures that stress test the limits of LLMs. 
Our approach leverages an A* search over a custom domain-specific language to produce complex story structures and novel, diverse, yet plausible scenarios to stress test the limits of LLMs. 
%, enabling effective evaluation and improvement of their theory of mind abilities. 
Our evaluation reveals that state-of-the-art LLMs, such as Llama-3.1-70B and GPT-4o, show accuracies as low as \finalnumber{0\%} and \finalnumber{9\%} on \methodname{}-generated data, highlighting the need for more robust theory of mind evaluation. As our generations are a conceptual superset of prior work, fine-tuning on our data yields a \finalnumber{27}-point accuracy improvement on the classic ToMi benchmark \citep{le2019revisiting}. %, demonstrating the effectiveness of our approach for both training and evaluation. 
\methodname{} also enables uncovering underlying skills and factors missing for models to show theory of mind, such as unreliable state tracking or data imbalances, which may contribute to models' poor~performance~on~benchmarks.%and a possible imbalance against theory of mind data in training data. 
\footnote{Code and data can be found at \url{https://github.com/facebookresearch/exploretom}.} % which could be contributing to poor performance on benchmarks


% \todo{Write the actual abstract}
% \bigskip
% .
% \bigskip
% .
% \bigskip
% .
% \bigskip
% .
% \bigskip
% .
% \bigskip
% .
% \bigskip
% .
% \bigskip
% .
% \bigskip
% .
% \bigskip
% .
% \bigskip
% .
% \bigskip
% .
% \bigskip

\end{abstract}

==> sections/introduction_v0.tex <==
\section{Introduction}

\begin{comment}
\begin{itemize}
\item Theory of Mind is X and it is important.
\item NLP research of ToM is centered mainly around evaluating the existence or not of ToM in models through eval benchmarks. Explicit ToM data is hard to find in the wild. Risk of leakage in training set, invalidates datasets. Risk of manually building a dataset that ends up being too easy for the model.
\item Some specific works focus on inference time algorithms (SymbolicToM) to improve performance. This might not be a good idea if you want to combine with other inference algorithms. Training for ToM was generally prohibitive given the lack of training data. 
\item OUR CONTRIBUTION: an adversarial and automatically generated dataset for ToM understanding. We guarantee accuracy. Rich in diversity. 
\item OUR CONTRIBUTION: Given the additional diversity wrt to prior work, we are able to scale generation to enable fine-tuning for tom. \todo{we thought of having automatic generation of CoT too, maybe for a follow-up? idk}
\end{itemize}
\end{comment}

\yejin{
NOTES FROM OUR 1:1

- 1st and 2nd paragraphs could be shortened
- 3rd reads as we're complaining that people faithfully evaluate; say: ``while there has been a lot of prior work that aim to eval tom in llms, conflicting results from prior research indicate that eval remains a major challenge, and training remains as another challenge'' 
``there have been a lot of prior resarch on tom benchmarks and speculation about how some of them are biased towards the familiar ToM tasks like Sally Anne, hence eval might be missing out variations of those classical cases where the models are actually much worse at (Ullman). This motivates the need for a method to systematically evaluate all corner cases for tom''

IDEA: Introduce your contributions earlier, trying to talk first about our work, and then explaining why it's different from others. This would reorder paragraphs 3 and 4 to appear later.
}

%\mel{Asli: there are missing things for the final submission, hidden with the command srtnotes. I am also using non-final data for the plots. I made this so that we can have them commented for the submission on Monday. I will continue tomorrow morning}
%\mel{The textbf in the intro are not going to be there in the final version, don't worry.}\asli{I like these summary sentences which are summarizing each paragraph :).}

%%%% 1. ToM reasoning is X, and it is important for social intelligence. LLMs should have it.
%\textbf{ToM reasoning is X, and it is important for social intelligence.}

Reasoning about other people's intentions, goals, thoughts, and beliefs is a foundation of social intelligence. Known as \textit{Theory of Mind (ToM)}~\citep{premack1978does}, the capability of reasoning about the mental states of others is crucial in human interaction: incorrectly predicting someone else's desires or knowledge may lead to a wrong estimation of their future actions, which in turn may entail a worse final result (e.g., in a negotiation), or delay task completion in a collaborative~setting.

% Theory of Mind (ToM) is the capability of reasoning about the mental states of others \citep{premack1978does}. It is crucial for interacting with other humans, and a key capacity for agents to be able to effectively interact and solve tasks in multi-agent scenarios. When an agent lacks theory of mind, they may incorrectly predict what the other agent wants or knows, leading to a wrong estimation of their future actions. This may delay task completion (e.g., a cooperative setting with partial observability for each agent), or lead to a worse final result (e.g., a worse outcome as a result of a negotiation). 

%\textbf{LLMs should have tom. explain how we test humans, and how just applying the tests leads to overestimation. Overestimation is bad.}
%%%% Mel: we probably want to add stuff here depending on flow needs
Large language models (LLMs) are increasingly being deployed in settings requiring human interaction, such as human-agent collaborative settings, or for multi-agent collaboration. In order to effectively collaborate, it is important to develop LLMs with robust ToM skills, as well as accurately characterize current LLMs' theory of mind abilities.

% However, theory of mind is largely an implicit reasoning skill learned in childhood in humans, and thus training data is hard to obtain, and evaluation data is limited. [...] \todo{Include whatever we may need for flow; we're missing the point of overestimating being bad, but maybe we don't need it. there is a small repetition with the paragraph below}

%[LLMs need ToM to interact with humans effectively. ToM is about implicit reasoning about mental states and intentions. We test ToM in humans with tasks like the Sally-Anne test [ref], and LLMs should be able to do the same, not just rely on surface-level cues. It's also important to be realistic when evaluating ToM capabilities of LLMs, because overestimating them can lead to mistakes and miscommunication.]
%\todo{connect with LLMs, emphasize implicit nature of ToM; emphasize reasoning, mention how this is tested in humans; emphasize why it is important to not overestimate perf}\asli{I gave it a shot, feel free to edit.} % Thank you! Took the idea of connecting LLMs

%%%% 2. Everyone focuses on benchmarking. web data to evaluate tom performance is hard to find. Current works on benchmarking ToM have issues.
%\textbf{Everyone focuses on benchmarking. web data to evaluate tom performance is hard to find. Current works on benchmarking ToM have issues.}
ToM research in LLMs has mainly centered on creating benchmarks to faithfully evaluate models' capabilities \citep[inter alia]{sap2022neural, shapira2023clever, fantom, t4d, bigtom}. Due to ToM's implicit nature, it is challenging to find data that explicitly articulates the required reasoning and/or isolates it for testing purpose. Therefore, researchers have developed cleverly crafted benchmarks inspired in tests from developmental psychology such as the Sally-Anne test \citep{wimmer1983beliefs}. These famous psychology tests---consisting of brief narratives (stories) with questions that probe understanding of each characters' mental state---are widely available online. As a result, models are likely to encounter them during training, potentially leading to an inadvertent overestimation of a model’s capabilities \citep{ullman2023large}.
%
Moreover, it is becoming increasingly harder to anticipate LLMs failures given their rapidly improving performance, which may lead to benchmarks already showing high theory of mind performance at the time of release (e.g., \cite{biggenbench}).
Finally, manually crafted benchmarks are the most exposed to leakage risks, as it would cause the whole work to be fully unusable for future benchmarking.

%%% Training data is impossible to get or limited in diversity
%\textbf{Training data is impossible to get or limited in diversity}
Existing ToM benchmarks are designed exclusively for evaluation purposes and are not suitable for training: they typically portray specific, scripted scenarios of human interaction, and are often limited in scale \citep{opentom}---particularly those that are manually curated.
%As a result, % of this, % lack of diversity and scale, 
Thus, there has been evidence of overfitting to specific story structures instead of learning the underlying reasoning required~\citep{symbolictom}.

%%%% Works on improving ToM at inference time are not a long term solution
%\textbf{Works on improving ToM at inference time are not a long term solution}
To bypass the issue of lack of diverse training data, some works have focused on creating inference-time algorithms to improve the model's capabilities through prompting or more sophisticated algorithms \citep{symbolictom, t4d, simtom, jung2024perceptions}
%\asli{we could cite strawberry/google's scaling LLM test time paper here?}\mel{oh I only included tom-ones but happy to cite more broadly!}. 
While inference-time methods have proven useful for improving performance in ToM benchmarks, they do not fundamentally improve the underlying language models' reasoning capabilities. As a result, the benefits of these methods cannot be readily transferred to downstream applications that may also require customized inference-time algorithms for their specific use cases.

\begin{figure}[]
    \centering
\includegraphics[width=\linewidth]{images_pdf/figure 1 track the mind isolated.pdf}
    \caption{\methodname{} finds challenging stories for a given language model by searching through the space of stories supported by its domain-specific language for mental state tracking~(\includegraphics[height=0.8em]{images_pdf/trackthemind-dsl-logo.pdf}), sampling $k$ supported actions at a time (shown as a node, $k=2$ in the example). Difficulty evaluation (simplified in the figure as \textcolor{easy}{easy}, \textcolor{medium}{medium}, \textcolor{hard}{hard}) of each partial story is done through automatically generated questions
    with reliable ground-truth answers %whose answers guaranteed to be correct 
    thanks to our tracking procedure. %Mental state questions may be about someone's beliefs about the world state (\textit{first-order} questions; see question \#3) or about someone's estimations of someone else's mental state (\textit{first-order} questions; see question \#4).\todo{Explain what false belief is here?}
    }
    \vspace{-0.5em}
    \label{fig:dsl}
\end{figure}

%\textbf{HIGH LEVEL CONTRIBUTION OF TTM: creates diverse stories (more supported actions than ever before). its automatic generation method guarantees the generations to be difficult for models, enabling its use as an evaluation benchmark or for training a better model. plausible contexts. automation and diversity implies well suited for training.}\\
We introduce \methodname{}, an A*-powered algorithm for generating reliable, diverse, and challenging ToM data. Building on standard approach in ToM of assessing mental state understanding through question-answering, \methodname{} significantly expands story diversity, allowing the generated data to be utilized as either a robust evaluation benchmark, or as scalable training data. Notably, \textbf{Llama-3.1 70B Instruct shows accuracies as low as \numbertbd{0.06} on \methodname{}-generated data}; % \mel{Here I need to talk about the avg performance as eval benchmark} Notably, 
and fine-tuned models leveraging \methodname{}'s data achieve a substantial \textbf{\numbertbd{+28} accuracy point on the classic ToMi benchmark}~\citep{le2019revisiting}. Furthermore, \methodname{}'s adversarial generation process ensures that its data is inherently challenging, thereby providing enhanced robustness to data leakage and enabling the stress testing of future models. 

% Reliable needs to come first because we need to explain DSL and what an action means
% Then we mention the adversarial part talking about figure 1
% Only then we talk about diversity and plausibility -- which also includes the infilling part.

To ensure reliability, we develop a domain-specific language (DSL) to generate synthetic story structures and their associated mental states, focusing solely on knowledge-related aspects. \jane{The previous clause feels a bit vague? (e.g., "knowledge related aspects"). Also not sure if I know what a DSL is and it doesn't seem like you use the term later in the paper.} We then leverage LLMs to create natural-looking stories based on these plots. Our approach allows for precise control over the narrative, tracking each character's mental state at every point of the story with a high degree of confidence. % Our approach allows for precise control over the narrative, 
% Our approach allows for precise control over the narrative, reducing the risk of data leakage and biases
% i don't think this is accurate, it's more about having more confidence about expected mental states
In addition, our DSL enables to systematically search for challenging stories that require robust ToM reasoning. To efficiently identify such stories, we use an A* search algorithm \citep{hart1968formal}, which is well-suited for navigating the vast space of possible narratives and pinpointing those that are most likely to elude or mislead state-of-the-art LLMs (Figure 1). By doing so, we create a robust and diverse dataset that effectively tests the limits of current models.
%\asli{I commented it and tried this above, please revise.} 
% \textbf{How is it reliable? DSL first. How are they difficult to solve? adversarial contribution}
% %We introduce \methodname{}, an algorithm for reliable synthetic story generation to facilitate theory of mind reasoning. 
% Reliable synthetic data is achieved by generating story structures, and all associated mental states (knowledge only) with a DSL. We will then use models to generate natural-looking stories from these plots.
% % \methodname{} ensures reliable data generation through the development of a domain-specific language for mental state tracking. 
% \todo{CONTINUE ON RELIABILITY}
% Furthermore, this domain-specific language enables adversarially finding difficult stories the adversarial discovery of stories that require theory of mind reasoning and are challenging for state-of-the-art LLMs to handle  using an A$^{\text{*}}$ search algorithm (Figure \ref{fig:dsl}). %\asli{we should use ToM or theory of mind, but not both. I am fine either way but lets choose one.} I'm trying to always use the full name throughout the text. If you see ToM without a reason, it's a bug!
%\mel{This paragraph still needs love}


%\textbf{Diversity and plausibility improvement} % \todo{asymmetry for the first time ever}
\methodname{} significantly enhances story diversity by supporting a wider range of actions than ever before, %.  Our framework supports a broad range of actions, 
including nuanced physical movements and verbal communication, as exemplified in Fig.~\ref{fig:dsl}. %previously available, such as location movements of objects and people, general object state updates, and verbal communication that conveys information about world states or casual conversation (e.g., chit-chat), all of which can occur in one-on-one or public settings.  %%% Mel: I would love to include this but the intro it way too long
% All sentences shown in Fig.~\ref{fig:dsl} exemplify supported actions. 
We also uniquely incorporate scenarios where characters have unequal access to information, such as one character secretly observing another or being distracted.  %% Jane mentioned we might want to remove this 
% We also uniquely include the possibility of \textit{asymmetry} in knowledge gain, e.g. having someone peeking in secret, or someone being distracted. 
Moreover, our story context sampling procedure ensures variety in story settings while our infilling procedure, aided by LLMs, generates linguistically diverse stories from story structures.
% Moreover, our stories are more linguistically diverse thanks to our infilling procedure that turns story structures into natural-sounding stories, and thanks to our story context sampling procedure, both LLM-aided.
%natuLLM-aidedral-looking than prior work thanks to  sampling plausible contexts using an LLM, and making the generated story structures appear more natural and linguistically diverse.
%
\srtnotes{
\textbf{Brain Dump} We will additionally automatically generate chain of thought rationales.}
%%%% Training data aspect
%\textbf{Training data aspect results?}
% This lack of training data makes progress in imbuing language models with ToM reasoning impossible. Thus, although inference-time methods proven useful for improving performance in ToM benchmarks, there is a need for imbuing language models with ToM skills that can then be leveraged for varied applications.
% Given the additional diversity \methodname{} supports, our generated data can be used both as an evaluation benchmark, or as training data to improve theory of mind reasoning in LLMs.
% we are able to scale generation to enable fine-tuning for theory of mind reasoning. \todo{Discuss reliability (or not) of our approach.}

%%%% Why is ToM hard still?
%\textbf{Why is ToM hard still?}
% \methodname{} also enables exploring why basic theory of mind is still difficult for language models. We show that empirically, random story generation is biased towards stories that do not require theory of mind, which may contribute to LLMs' low performance. Finally, using \methodname{} we show that frontier LLMs still struggle with basic state tracking---an easier, underlying skill required for the kind of theory of mind tests developed in this work.
By leveraging \methodname{}, we uncover new insights into why basic ToM reasoning is still challenging for LLMs. Our empirical analysis reveals that random story generation tends to produce narratives that do not require ToM, which may contribute to the low performance of LLMs on ToM tasks. Furthermore, our results show that even state-of-the-art LLMs struggle with basic state tracking, a fundamental skill underlying ToM reasoning. This finding highlights the need for more sophisticated ToM benchmarks and training data, which \methodname{} is designed to provide.
\srtnotes{\asli{can we inlcude concrete results in the last two paragraphs based on the benchmarks?}\mel{good point! I still don't have the numbers for state tracking; we'll add it for the final submission}}

% \asli{Observations on Introduction: (1) I know this is just a draft but i think the story is a tad mixed-up. It started well but we need to emphasize the contribution of TrackTheMind in a more organized fashion. I can help here. (2)Figure 1 is A* search, Figure 2 (which is amazing) is TrackTheMind process. I wonder if we first present the process then talk about the A* search. Maybe once we write the intro better we can decide on this. }\mel{I think Figure 2 is too much detail for the intro, I'm trying to make Figure 1 a selling point for people to be interested on the technical novelty. I fear Figure 2 will sound too boring as the first thing shown about the paper...}
% gave another stab to the intro, we need to shorten it---I'm listing every single novelty aspect which may be too much

==> sections/introduction_v1_asli.tex <==
\section{Introduction}

\todo{This is Asli's revision of the intro ; I think we could add back some more motivation since we're saving so much space now!}
\mel{Some things that are currently missing to add back for future edits if space allows:\\
- motivation on why training data is hard to find and no mention of prior work overfitting; or why training is important. I think we should bring this back.\\
- mention of the analysis of what makes tom hard\\
- I think we should mention HOW we expand story diversity (more actions; unique additions like asymmetry and linguistic diversity)
- Should we explain what ToM tests are usually like? and that we follow them? (unsure)
}

Reasoning about other people's intentions, goals, thoughts, and beliefs is a foundation of social intelligence. %, known as \textit{Theory of Mind (ToM)}~\citep{premack1978does}.  
\editmel{Known as \textit{Theory of Mind (ToM)}~\citep{premack1978does}, this capability is crucial for effective human interaction.} %to avoid wrong estimation of other people's future actions, which in turn may entail a worse final result (e.g., in a negotiation), or delay task completion in a collaborative~setting.} %%% Mel this is too much fluff still but I fear we need *SOMETHING*
%
\editmel{As Large Language Models (LLMs) are increasingly being deployed in settings requiring it---such as human-agent collaborative settings, or for multi-agent collaboration---imbuing LLMs with robust theory of mind skills and faithfully assessing theory of mind skills is becoming ever more crucial.} % \citep[inter alia]{sap2022neural, shapira2023clever, fantom}. \editmel{However, LLMs still lack robust theory of mind skills.}

We introduce \textbf{\methodname{}}, an A*-powered algorithm for generating reliable, diverse, and challenging theory of mind data\editmel{, and can be effectively employed as test data or fine-tuning data}. Our approach leverages a domain-specific language (DSL) to generate synthetic story structures and their associated mental states, focusing solely on knowledge-related aspects. We then use LLMs to create natural-looking stories based on these plots, allowing for precise control over the narrative and tracking each character's mental state with high confidence. We employ A*-search~\citep{hart1968formal} to efficiently navigate the vast space of possible narratives and pinpoint those that are most likely to elude or mislead state-of-the-art LLMs. This in turn allows to create a robust and diverse dataset that effectively tests the limits of current models (Figure~\ref{fig:dsl}).

While there has been significant prior work on creating benchmarks to evaluate theory of mind in LLMs~\citep[inter alia]{sap2022neural, shapira2023clever, fantom, t4d, bigtom}, conflicting results from prior research indicate that faithful evaluation remains a major challenge, and \editmel{robust theory of mind skills are still lacking}%training remains another challenge
~\citep{ullman2023large}. Existing benchmarks are often limited in scale~\citep{opentom}, portray specific scripted scenarios~\citep{hitom, le2019revisiting}, and are prone to leakage risks\editmel{ that would make them fully unsuitable for future use}. %Moreover, manually crafted benchmarks may inadvertently overestimate a model's capabilities due to the rapidly improving performance of LLMs (e.g.,~\cite{biggenbench}). % Mel: commenting this one because I think it's important to explain what we mean by overestimation; these are not mislabels.
\editmel{Moreover, benchmarks may already be close to saturation at the time of release, given that it is becoming increasingly harder to anticipate LLMs failures (e.g., \cite{biggenbench}).}

\begin{figure}[t]
    \centering
\includegraphics[width=\linewidth]{images_pdf/figure 1 track the mind isolated.pdf}
    \caption{\methodname{} finds challenging stories for a given language model by searching through the space of stories supported by its domain-specific language for mental state tracking~(\includegraphics[height=0.8em]{images_pdf/trackthemind-dsl-logo.pdf}), sampling $k$ supported actions at a time (shown as a node, $k=2$ in the example). Difficulty evaluation (simplified in the figure as \textcolor{easy}{easy}, \textcolor{medium}{medium}, \textcolor{hard}{hard}) of each partial story is done through automatically generated questions
    with reliable ground-truth answers %whose answers guaranteed to be correct 
    thanks to our tracking procedure. %Mental state questions may be about someone's beliefs about the world state (\textit{first-order} questions; see question \#3) or about someone's estimations of someone else's mental state (\textit{first-order} questions; see question \#4).\todo{Explain what false belief is here?}
    }
    \vspace{-0.5em}
    \label{fig:dsl}
\end{figure}

In contrast, \methodname{} significantly expands story diversity, allowing the generated data to be utilized as either a robust evaluation benchmark or scalable training data. We demonstrate the effectiveness of \methodname{} through experiments, showing that \textbf{Llama-3.1 70B Instruct achieves as low as 0.06 accuracy on \methodname{}-generated data, and fine-tuned models leveraging \methodname{}'s data achieve a substantial +28 accuracy point improvement on the classic ToMi benchmark}~\citep{le2019revisiting}. Our approach ensures reliability, provides enhanced robustness to data leakage, and enables the stress testing of future models.


% \begin{figure}[]
%     \centering
% \includegraphics[width=\linewidth]{images_pdf/figure 1 track the mind isolated.pdf}
%     \caption{\small \methodname{} finds challenging stories for a given language model by searching through the space of stories supported by its domain-specific language for mental state tracking~(\includegraphics[height=0.8em]{images_pdf/trackthemind-dsl-logo.pdf}), sampling $k$ supported actions at a time (shown as a node, $k=2$ in the example). Difficulty evaluation (simplified in the figure as \textcolor{easy}{easy}, \textcolor{medium}{medium}, \textcolor{hard}{hard}) of each partial story is done through automatically generated questions
%     with reliable ground-truth answers %whose answers guaranteed to be correct 
%     thanks to our tracking procedure. %Mental state questions may be about someone's beliefs about the world state (\textit{first-order} questions; see question \#3) or about someone's estimations of someone else's mental state (\textit{first-order} questions; see question \#4).\todo{Explain what false belief is here?}
%     }
%     \vspace{-0.5em}
%     \label{fig:dsl}
% \end{figure}

==> tables/table_accuracy_all_settings.tex <==
\begin{table}[t]
\centering
\caption{Accuracy results of  \methodname{}'s story structures on various action sets $\mathcal{A}$, aggregating all settings (number of people, actions, and rooms). Each set is either based on actions supported by well-known ToM tests or includes our novel expansions, and is analyzed excluding or including asymmetry (\xmark{}, \cmark{}). Data was generated using each model as its own evaluator (i.e., as $g(\cdot)$).% \asli{what does X and check mark mean in under each model? Also, will we have GPT-4 and Mixral results by Monday?} \mel{They say whether we add asymmetry or not, I thought it looked nicer than yes/no}
\srtnotes{These are the numbers from our random baseline generations, which for some reason look better than my other numbers. I am debugging why this is happening, I think it's just that I used a bigger budget but I will check after Monday.}}\label{tab:eval_benchmark_accuracy}
\begin{tabular}{@{}ccccccc@{}}
\toprule
\begin{tabular}[c]{@{}c@{}}\methodname{} action set \\ $\{a_{\text{enter}}, a_{\text{leave}}, \ldots$\end{tabular} & \multicolumn{2}{c}{\begin{tabular}[c]{@{}c@{}}Llama-3.1 \\ 70B Chat\end{tabular}} & \multicolumn{2}{c}{\begin{tabular}[c]{@{}c@{}}GPT-4\end{tabular}} & \multicolumn{2}{c}{\begin{tabular}[c]{@{}c@{}}Mixtral\end{tabular}}   \\ \midrule
include asymmetry modifiers? ($a_{\text{peek}}$, $a_{\text{distracted}}$) & \xmark & \cmark
 & \xmark & \cmark
  & \xmark & \cmark
 \\ \midrule \toprule
% ['tomi', 'tomi-object-state', 'tomi+object-state', 'tomi+room-changes', 'tomi+info-exchange', 'tomi+room-changes+info-exchange', 'tomi+fantom+room-changes+info-exchange', 'fantom-private', 'fantom-public']
% tomi 
$\ldots, a_{\text{moveObjContainer}}\}$ & 0.31 & 0.12 & & & & \\
% tomi-object-state
$\ldots, a_{\text{updateObjState}}\}$ & 0.38 & 0.06 & & & & \\
% tomi+object-state 
$\ldots, a_{\text{moveObjContainer}}, a_{\text{updateObjState}}\}$  & 0.31 & 0.21 & & & & \\
% tomi+room-changes
$\ldots, a_{\text{moveObjRoom}}\}$ & 0.37 & 0.14 & & & & \\
% tomi+info-exchange 
$\ldots, a_{\text{moveObjContainer}}, a_{\text{info-*}}\}$
& 0.34 & 0.23 & & & & \\
% tomi+room-changes+info-exchange 
$\ldots, a_{\text{moveObjContainer}}, a_{\text{moveObjRoom}}, a_{\text{info-*}} \}$
& 0.35 & 0.13  & & & & \\
% tomi+fantom+room-changes+info-exchange 
$\ldots, a_{\text{moveObjContainer}}, a_{\text{moveObjRoom}}, a_{\text{chitChat-*}}, a_{\text{info-*}} \}$
& 0.40 & 0.10 & & & & \\
% fantom-private 
$\ldots, a_{\text{chitChat-private}} \}$ & 0.75 & 0.42 & & \\
% fantom-public 
$\ldots, a_{\text{chitChat-public}} \}$ & 0.78 & 0.40 & & \\
\bottomrule
\end{tabular}
\end{table}

